Residual supersingular Iwasawa theory and signed Iwasawa invariants

For an odd prime $p$ and a supersingular elliptic curve over a number field, this article introduces a fine signed residual Selmer group, under certain hypotheses on the base field. This group depends purely on the residual representation at $p$, yet captures information about the Iwasawa theoretic invariants of the signed $p^\infty$-Selmer group that arise in supersingular Iwasawa theory. Working in this residual setting provides a natural framework for studying congruences modulo $p$ in Iwasawa theory.

==> arxiv_preamble_v4.tex <==
\makeatletter
%%%Typographical packages and commands
\usepackage[sc]{mathpazo}
\usepackage{eucal}
\usepackage{verbatim}
\usepackage{mathrsfs}
\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
\DeclareSymbolFontAlphabet{\mathbbold}{bbold}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[left=2.5cm,right=2.5cm]{geometry}
\usepackage[english]{babel}
\hyphenation{Le-mma}
\usepackage[dvipsnames]{xcolor}
\usepackage[colorlinks=true,linkcolor=Emerald,citecolor=Emerald]{hyperref}
\usepackage{cancel}
\usepackage{soul}
\usepackage{subcaption}
%\usepackage[notref,notcite,color]{showkeys}
%\newcommand{\fil}[1]{{\color{red}#1}}
\newcommand{\suj}[1]{{\color{blue}#1}}
%\newcommand{\suj}[1]{#1}
\newcommand{\here}[1]{\par \bigskip \begin{center} {\LARGE\color{brown}\textsc{Arrived here on #1}}\bigskip\end{center}}
\newcommand{\resp}{\emph{resp.}\kern.3em}
%%%%Math packages
\usepackage{amsmath,amsthm,amssymb}
\usepackage{mathtools}
\usepackage{enumitem}
\usepackage[all]{xy}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%Theorems%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\numberwithin{equation}{subsection}
\newcounter{eqPM}
\newtheorem{proposition}{Proposition}[section]
\newtheorem{theorem}[proposition]{Theorem}
\newtheorem{lemma}[proposition]{Lemma}
\newtheorem{corollary}[proposition]{Corollary}
\newtheorem*{c@njecture}{\conjn@name}
\newcommand{\myl@bel}[2]{%
   \protected@write \@auxout {}{\string \newlabel {#1}{{#2}{\thepage}{#2}{#1}{}} }%
   \hypertarget{#1}{}
	}
\newenvironment{labelledconj}[3][]%
	{
		\def\conjn@name{#2}
		\begin{c@njecture}[{#1}]\myl@bel{#3}{#2}
	}
	{
		\end{c@njecture}
	}
\newtheorem*{intr@thm}{\intr@thmname}
\newenvironment{introtheorem}[1]{%
	\def\intr@thmname{Theorem #1}
	\begin{intr@thm}}
	{\end{intr@thm}}
\theoremstyle{definition}
\newtheorem{definition}[proposition]{Definition}
\theoremstyle{remark}
\newtheorem{remark}[proposition]{Remark}
\newtheorem{notation}[proposition]{Notation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%Math Commands%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%Main Objects
\def\gener@alfield{K} %The generic field
\def\b@se{\mathrm{L}} %The base field
\def\loc@l{\mathcal{L}} %The base local field
\def\cycl@loc{\Bbbk} %The cyclotomic local field
\def\prim@set{\ensuremath{S}} %The set of primes
%%%%%%%%%%%%%%
\newcommand*{\tors}[2]{#1_{#2}} %The #1-torsion of #2
\DeclareMathOperator{\image}{Im} %Image of a morphism
\DeclareMathOperator{\Hom}{Hom} %Hom functor
\DeclareMathOperator{\Ext}{Ext} %Ext functor
\DeclareMathOperator{\coker}{coker} %Cokernel of a morphism
\DeclarePairedDelimiterXPP{\Gal}[2]{\mathrm{Gal}}{(}{)}{}{#1/#2} %%Galois group of #1 over #1
\newcommand*{\QQ}{\mathbb{Q}} %Rational field
\newcommand*{\ZZ}{\mathbb{Z}} %Rational integers
\newcommand*{\NN}{\mathbb{N}} %Natural numbers
\newcommand*{\primeset}[1][\empty]{\prim@set_{{#1}}} %The Set S of primes
\newcommand*{\ssprimeset}[1][\empty]{\prim@set^\mathrm{ss}_{#1}} %The Set Sp^ss of d suspersingular (p)-adic primes
\newcommand*{\ordssprimeset}{d}
\newcommand*{\ordprimeset}[1][\empty]{\prim@set^\mathrm{ord}_{#1}} %The Set S_p^ord of s ordinary (p)-adic primes
\newcommand*{\ordordprimeset}[1][\empty]{s_{#1}}
\newcommand*{\pprimeset}{\prim@set_p} %The Set S_p p-adic primes
\newcommand*{\badprimeset}[1][\empty]{\prim@set^\mathrm{bad}_{#1}} %The Set S^bad of r bad primes
\newcommand*{\ordbadprimeset}[1][\empty]{r_{#1}}
\newcommand*{\genprimeset}[1][\empty]{\prim@set^\ast_{#1}} %Any of the above sets S of primes
\newcommand*{\ordcycprimes}[1]{g_{#1}} %The number of primes in Lcyc above #1
\newcommand*{\galprime}{\Delta} %The Galois group isomorphic to Z/(p-1) of Q(\zeta_p)/Q
\newcommand*{\cyc}{\mathrm{cyc}}
\newcommand*{\Qcyc}{\mathbb{Q}^\cyc} %Cyclotomic Z_p-extension of Q
\newcommand*{\QS}{\mathbb{Q}_{\prim@set}} %Maximal S-ramified extension of Q
%...
\newcommand*{\basefield}[1][]{{\b@se_{#1}}} %The GLOBAL field F_#1, which is the #1-th layer of the Z_p cyclotomic extension of F=\basefield
\newcommand*{\degbase}{N}
\newcommand*{\basecyc}[1][\@empty]{%
	\ifx\@empty#1 \basefield_{\cyc}
	\else \basefield_{\cyc,#1}
\fi} %Cyclotomic Z_p-extension of the base field
\newcommand*{\baseS}{\basefield^{\prim@set}} %Maximal S-ramified extension of the base field
\newcommand*{\baseSloc}[1]{(\basefield^{\prim@set})_{#1}} %Localization at #1 of the maximal S-ramified extension of the base field
\newcommand*{\GS}[1][]{\mathscr{G}^\prim@set_{#1}} %The Galois group of \baseS/basefield[n]; if no variable, of \baseS/\base; use n=\infty for \baseS/\basecyc.
%\newcommand*{\ideleS}[2][\prim@set]{\mathcal{C}_{#2,#1}} %The \primeset-ramified Idèle Classes of #1.
%\newcommand*{\NSWI}[2][\prim@set]{\mathcal{I}_{#2,#1}} %The \primeset-ramified Idèle Classes of #1.
\newcommand*{\localfield}[2][\@empty]{ %%The n-stage of the cyclotomic extension of Q_p. The optional variable gives ^{(i)}, to distinguish among the d primes above p in \basefield.
	\ifx\@empty#1 \loc@l_{#2}
	\else 		\loc@l_{#2,#1}
	\fi
} 
\newcommand*{\ssloccyc}[1][\@empty]{
	\ifx\@empty#1 \loc@l_{\cyc}
	\else 		\loc@l_{\cyc,#1}
	\fi}
 %Cyclotomic Z_p-extension of the local field Q_p (should it become \Q_p^{cyc}?)
\newcommand*{\fullcyc}[1]{\cycl@loc_{#1}} %The "full" cyclotomic extension QQ_p(\zeta_p^n)
\newcommand*{\cyclocal}[2][1]{\genlocal{#2}^{#1}} %The #1-th layer of the cyclotomic extension of the local field at #2.
\newcommand*{\genlocal}[2][\@empty]{
	\ifx\@empty#1 \b@se_{#2}
	\else 		\b@se_{#1, #2}
	\fi} %The ``generic'' local field at #2; the second option gives the localization of base[#1] at #2
\newcommand*{\locbar}{\overline{\QQ_p}} %A (fixed?) algebraic closure of QQ_p
%\newcommand*{\Glocal}[1][0]{G_{\localfield{#1}}} %The Galois group of \overline{local}/local{n}; if no variable, of overline{local}/local; use n=\cyc for \overline{local}/local{\cyc}
\newcommand*{\Glocal}[2][\localfield]{G_{#1{#2}}} %The Galois group of \overline{local}/local{n}; if no variable, of overline{local}/local; use n=\cyc for \overline{local}/local{\cyc}
%%%%%%%%% Useful: the generic local absolute Galois group is $\Glocal[{\genlocal[n]}]{\genprimeid}$
\newcommand*{\Gv}[1]{G_{#1}} %The absolute Galois group of the localization of \basefield at #1; only have it for basefield
\newcommand*{\field}{\gener@alfield} %The GENERIC field L_#1
\newcommand*{\fieldcyc}{\gener@alfield_\cyc} %Its cyclotomic extension
\newcommand*{\fieldS}{\widetilde{\gener@alfield}} %Its algebraic/S closure
\def\finit@field{\mathbb{F}}
\newcommand*{\finitefield}[1][p]{\finit@field_{#1}}
\def\int@gers{\mathcal{O}}
\newcommand*{\rootsp}[1][p]{\mathbbold{\mu}_{#1}}
\newcommand*{\rint}[1]{\int@gers_{#1}} %%The ring of integers of the field (#1)
\def\m@ximal{\mathfrak{m}} 
\newcommand*{\maxid}[1]{\m@ximal_{#1}} %%The maximal ideal of the local field k_{#1}
\def\ssprim@{\mathfrak{p}}
\newcommand*{\ssprimeid}[2][\@empty]{ %%The (#2)-th prime ideal above p of the (#1)-th cyclotomic layer of basefield=maximal ideal of the local field k_{#2}^{(#1)}. By default of the basefield.
	\ifx\@empty#1 \ssprim@_{#2}
	\else 		\ssprim@_{#1,#2}
	\fi
} 
\def\ordprim@{\pi}
\newcommand*{\ordprimeid}[2][\@empty]{ %%The (#2)-th prime ideal above p of the (#1)-th cyclotomic layer of basefield=maximal ideal of the local field k_{#2}^{(#1)}. By default of the basefield.
	\ifx\@empty#1 \ordprim@_{#2}
	\else 		\ordprim@_{#1,#2}
	\fi
} 
\def\badprim@{\mathfrak{l}}
\newcommand*{\badprimeid}[2][\@empty]{ %%The (#2)-th prime ideal above p of the (#1)-th cyclotomic layer of basefield=maximal ideal of the local field k_{#2}^{(#1)}. By default of the basefield.
	\ifx\@empty#1 \badprim@_{#2}
	\else 		\badprim@_{#1,#2}
	\fi
}
\newcommand*{\BadPrimeId}[2][\@empty]{ %%The (#2)-th prime ideal above p at the cyclotomic level of basefield=maximal ideal of the local field k_{#2}^{(#1)}. By default of the basefield.
	\ifx\@empty#1 \mathfrak{q}_{#2}
	\else 		\mathfrak{q}_{#1,#2}
	\fi
} 
\newcommand*{\genprimeid}[1][\@empty]{ %%The generic prime ideal above p of the (#1)-th cyclotomic layer of basefield=maximal ideal of the local field k_{#2}^{(#1)}. By default of the basefield.
	\ifx\@empty#1 {v}
	\else 		{v}_{#1}
	\fi
} 
\newcommand*{\GenPrimeId}[1][\@empty]{ %%The generic prime ideal above p of the (#1)-th cyclotomic layer of basefield=maximal ideal of the local field k_{#2}^{(#1)}. By default of the basefield.
	\ifx\@empty#1 {w}
	\else 		{w}_{#1}
	\fi
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%Curves
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\curv@{E} %The name of our elliptic curve
\def\gencurv@{A} %The name of another generic elliptic curve
\def\curvef@nt{\mathsf} %The font for the elliptic curve
\def\formalf@nt{\mathcal} %The font for formal groups
\def\neronf@nt{\mathscr} %The font for Neron models
\newcommand*{\EC}{\curvef@nt{\curv@}} % The curve E
\newcommand*{\genEC}{\curvef@nt{\gencurv@}} %A generic curve different from the above
\newcommand*{\modEC}{\widetilde{\EC}} %The closed fiber of the curve, so its reduction modulo the prime ideals (no matter which one)
\newcommand*{\multisign}{\ddagger} %The vector of multi-signs
\newcommand*{\pmEC}[1][\pm]{\EC^{#1}} %E^\pm, by default; as an option, can be modified to sharp/flat or + or -, etc.
\newcommand*{\formalEC}{\formalf@nt{\curv@}} %The formal group attached to the curve
\newcommand*{\neron}{\neronf@nt{\curv@}} %The Néron model over Z_p
\newcommand*{\ordformalEC}{\formalf@nt{\gencurv@}} %The formal group attached to the curve at ordinary primes
\newcommand*{\pmformalEC}[1][\pm]{\formalEC^{#1}} %The pm-formal group attached to the curve
\newcommand*{\grpsch}{\neronf@nt{G}} %The formal group scheme over Z_p
\newcommand*{\pmMod}[2][\pm]{\formalf@nt{D}^{#1}_{#2}} %The equivalent of \pmEC but in the special fiber
\newcommand*{\tate}[2][p]{T_{#1}(#2)} %The p-adic Tate module of #2 (p=#1)
%\DeclarePairedDelimiterXPP{\tors}[2]{#1}{[}{]}{}{#2} %The #1-torsion of #2
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%MORE ALGEBRA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand*{\pontr}[1]{{#1}^{\land}} %The Pontryagin dual of the module #1
\newcommand*{\fullKum}[2]{\kappa_{#1}^{#2}} %The full Kummer map for the module E[#2] and the field #1 (NO ABBREVIATION WHATSOEVER IN PLACE OF #1!)
\newcommand*{\pmKum}[3][\pm]{\kappa^{#1,#3}_{#2}} %The pm-Kummer map for the module E[#3] and the field #2 (NO ABBREVIATION WHATSOEVER IN PLACE OF #2!)
\newcommand*{\fakeKum}[2][\@empty]{ %The fake Kummer morphism
	\ifx\@empty#1 {\psi_{#2}}
	\else 		{\psi_{#1,#2}}
	\fi
} 
\newcommand*{\modfakeKum}[2][\@empty]{ %The residual fake Kummer morphism
	\ifx\@empty#1 {\widetilde{\psi_{#2}}}
	\else 		{\widetilde{\psi_{#1,#2}}}
	\fi
} 
\newcommand*{\pmfakeKum}[2][\@empty]{ %The signed fake Kummer morphism
	\ifx\@empty#1 {\psi^{\pm}_{#2}}
	\else 		{\psi^{\pm}_{#1,#2}}
	\fi
} 
\newcommand*{\JJ}[2][\pm]{J^{#1}_{#2}({\tors{\EC}{p^\infty}}/\basecyc)} %Coates--Sujatha local conditions J_v
\newcommand*{\modJJ}[1][\pm]{\def\segn@{{#1}}\m@dJJ} %the residual local conditions J_v
\newcommand{\m@dJJ}[2][\tors{\EC}{p}]{{^{\segn@}\widetilde{K}}_{#2}({#1}/\basecyc)}

\newcommand*{\fullambda}[2]{\xi_{#2}} %The "full" map \lambda (as in Coates-Sujatha's book, eq. (4)) for the module E[#2] and the field #1
\newcommand*{\pmlambda}[3][\multisign]{\xi^{#1}_{#3}} %The pm-morphism \lambda for the module E[#3] and the field #2
\newcommand*{\plocallambda}[1]{\vartheta^{\multisign}_{#1,\pprimeset}} %The composition of \lambda for the module E[#3] and the field #2 at ordinary primes
\newcommand*{\localpmlambda}[3][\pm]{\vartheta^{#1}_{#3,#2}} %OLD The pm-morphism \lambda for the module E[#3] and the field #2
\newcommand*{\sspmlambda}[3][\pm]{\vartheta^{#1}_{#3,#2}} %The pm-morphism \lambda for the module E[#3] and the field #2
\newcommand*{\Fss}{\formalf@nt{F}_\mathrm{ss}} %The "supersingular" formal group
\newcommand*{\formalKO}{\formalf@nt{G}} %The formal group in Kitajima-Otsuki
\newcommand*{\pmFss}[1][\pm]{\Fss^{#1}} %The "pm-subgroup" of the supersingular formal group
\newcommand*{\Css}{\formalf@nt{C}_{\mathrm{ss}}} %The "pm-subgroup" of the supersingular formal group
\DeclarePairedDelimiterXPP{\fullSel}[2]{\operatorname{Sel}}{(}{)}{}{#1/#2} %Full Selmer group of the module #1 over the field #2
\DeclarePairedDelimiterXPP{\dualfineSel}[2]{\mathcal{Y}}{(}{)}{}{#1/#2} %Dual fine Selmer group of the module #1 over the field #2, in Coates-Sujatha's MathAnnalen notation
\DeclarePairedDelimiterXPP{\dualSel}[2]{\operatorname{X}}{(}{)}{}{#1/#2} %Dual Selmer group of the module #1 over the field #2
%A long command for signed Selmer groups, signed dual Selmer groups and signed compact Selmer groups starting here...
\DeclarePairedDelimiterXPP{\Selm@r}[2]{\s@lmerName}{(}{)}{}{#1/#2} %...
\newcommand{\S@l}[3][\multisign]{ %...
\def\s@lmerName{\mathcal{R}^{#1}} %...
\def\m@dule{#2} %...
\def\fi@ld{#3} %...
\Selm@r{\m@dule}{\fi@ld} %...
}%...
\newcommand{\S@@l}[3][\multisign]{ %...
\def\s@lmerName{\mathcal{R}^{#1}} %...
\def\m@dule{#2} %...
\def\fi@ld{#3} %...
\Selm@r*{\m@dule}{\fi@ld} %...
}%% So far, our fine signed Selmer
\DeclarePairedDelimiterXPP{\cptSelm@r}[2]{\cpts@lmerName}{(}{)}{}{#1/#2} %...
\newcommand{\cptS@l}[3][\multisign]{ %...
\def\cpts@lmerName{\mathfrak{R}^{#1}} %...
\def\m@dule{#2} %...
\def\fi@ld{#3} %...
\cptSelm@r{\m@dule}{\fi@ld} %...
}%...
\newcommand{\cptS@@l}[3][\multisign]{ %...
\def\cpts@lmerName{\mathfrak{R}^{#1}} %...
\def\m@dule{#2} %...
\def\fi@ld{#3} %...
\cptSelm@r*{\m@dule}{\fi@ld} %...
}%% So far, the Cassels-Poitout-Tate dual of our fine signed Selmer
\DeclarePairedDelimiterXPP{\KobSelm@r}[2]{\Kobs@lmerName}{(}{)}{}{#1/#2} %...
\newcommand{\KobS@l}[3][\multisign]{ %...
\def\Kobs@lmerName{\operatorname{Sel}^{#1}} %...
\def\m@dule{#2} %...
\def\fi@ld{#3} %...
\KobSelm@r{\m@dule}{\fi@ld} %...
}%...
\newcommand{\KobS@@l}[3][\multisign]{ %...
\def\Kobs@lmerName{\operatorname{Sel}^{#1}} %...
\def\m@dule{#2} %...
\def\fi@ld{#3} %...
\KobSelm@r*{\m@dule}{\fi@ld} %...
}%% So far, the classical signed Selmer à la Kobayashi
\newcommand{\dualS@l}[3][\multisign]{ %...
\def\s@lmerName{\operatorname{Y}^{#1}} %...
\def\m@dule{#2} %...
\def\fi@ld{#3} %...
\Selm@r{\m@dule}{\fi@ld} %...
}%...
\newcommand{\dualS@@l}[3][\multisign]{ %...
\def\s@lmerName{\operatorname{Y}^{#1}} %...
\def\m@dule{#2} %...
\def\fi@ld{#3} %...
\Selm@r{\m@dule}{\fi@ld} %...
}%% So far, our fine Dual Selmer
\newcommand{\KobdualS@l}[3][\multisign]{ %...
\def\s@lmerName{\operatorname{X}^{#1}} %...
\def\m@dule{#2} %...
\def\fi@ld{#3} %...
\Selm@r{\m@dule}{\fi@ld} %...
}%...
\newcommand{\KobdualS@@l}[3][\multisign]{ %...
\def\s@lmerName{\operatorname{X}^{#1}} %...
\def\m@dule{#2} %...
\def\fi@ld{#3} %...
\Selm@r{\m@dule}{\fi@ld} %...
}%% So far, the dual of Kobayashi's signed Selmer
\newcommand{\projS@l}[3][\multisign]{ %...
\def\s@lmerName{\mathscr{R}^{#1}} %...
\def\m@dule{#2} %...
\def\fi@ld{#3} %...
\Selm@r{\m@dule}{\fi@ld} %...
}%...
\newcommand{\projS@@l}[3][\multisign]{ %...
\def\s@lmerName{\mathscr{R}^{#1}} %...
\def\m@dule{#2} %...
\def\fi@ld{#3} %...
\Selm@r{\m@dule}{\fi@ld} %...
}%...
%%So far, the residual compact Selmer
\newcommand{\cptK@b}[3][\multisign]{ %...
\def\cpts@lmerName{\mathfrak{S}^{#1}} %...
\def\m@dule{#2} %...
\def\fi@ld{#3} %...
\cptSelm@r{\m@dule}{\fi@ld} %...
}%...
\newcommand{\cptK@@b}[3][\multisign]{ %...
\def\cpts@lmerName{\mathfrak{S}^{#1}} %...
\def\m@dule{#2} %...
\def\fi@ld{#3} %...
\cptSelm@r*{\m@dule}{\fi@ld} %...
}%% So far, the Cassels-Poitout-Tate dual of Kobayashi, so isomorphic to the Selmer of the Tate module
\newcommand{\KobprojS@l}[3][\multisign]{ %...
\def\s@lmerName{\mathscr{S}^{#1}} %...
\def\m@dule{#2} %...
\def\fi@ld{#3} %...
\Selm@r{\m@dule}{\fi@ld} %...
}%...
\newcommand{\KobprojS@@l}[3][\multisign]{ %...
\def\s@lmerName{\mathscr{S}^{#1}} %...
\def\m@dule{#2} %...
\def\fi@ld{#3} %...
\Selm@r{\m@dule}{\fi@ld} %...
}%...
%%So far, Kobayashi's compact Selmer
%%%%%And finally the definitions:
\def\pmSel{\@ifstar\S@l\S@@l} %The command \pmSel gives R^\pm(#1/#2). There is an optional argument to modify \pm into \sharp, \flat or other; and a starred version, avoiding "big" parenthesis.
\def\dualpmSel{\@ifstar\dualS@l\dualS@@l} %The command \dualpmSel gives Y^\pm(#1/#2). There is an optional argument to modify \pm into \sharp, \flat or other; and a starred version, avoiding "big" parenthesis.
\def\CPTSel{\@ifstar\cptS@l\cptS@@l} %The command \dualpmSel gives R^{\vert,\pm(#1/#2)}. There is an optional argument to modify \pm into \sharp, \flat or other; and a starred version, avoiding "big" parenthesis: CPT=Cassels-Poitou-Tate
\def\CPTprojlim{\@ifstar\projS@l\projS@@l} %This is \mathscr{S}: the projective limit of \CPTSel
\def\KobSel{\@ifstar\KobS@l\KobS@@l} %The command \KobSel gives Sel^\pm(#1/#2). There is an optional argument to modify \pm into \sharp, \flat or other; and a starred version, avoiding "big" parenthesis.
\def\KobdualSel{\@ifstar\KobdualS@l\KobdualS@@l} %The command \KobdualpmSel gives X^\pm(#1/#2). There is an optional argument to modify \pm into \sharp, \flat or other; and a starred version, avoiding "big" parenthesis.
\def\KobCPT{\@ifstar\cptK@b\cptK@@b}
\def\KobprojSel{\@ifstar\KobprojS@l\KobprojS@@l} %The command \pmSelprojlim gives \mathcal{R}^\pm(#1/#2), which is the compact Selmer of T_pE instead of E (defined using prohective limits). There is an optional argument to modify \pm into \sharp, \flat or other; and a starred version, avoiding "big" parenthesis.
%%%...and finishing here
\DeclarePairedDelimiterXPP{\HH}[3]{\operatorname{H}^{#1}}{(}{)}{}{#2,#3} %H^i: The convention is to use étale cohomology notation for local fields, where the Galois group is the absolute one; and to use group-cohomology notation for global fields, where the Galois group is G^S. When G can be either local or global, use group cohomology.
\DeclarePairedDelimiterXPP{\pmHH}[4]{\operatorname{H}_{#1}^{#2}}{(}{)}{}{#3,#4} %Plus/minus H^i 
\DeclarePairedDelimiterXPP{\HHiw}[3]{\operatorname{H}^{#1}_\mathrm{Iw}}{(}{)}{}{#2,#3} %Iwasawa H^i: The convention is to use étale cohomology notation for local fields, where the Galois group is the absolute one; and to use group-cohomology notation for global fields, where the Galois group is G^S. When G can be either local or global, use group cohomology.
\DeclarePairedDelimiterXPP{\pmHHiw}[4]{\operatorname{H}^{#2}_{#1,\mathrm{Iw}}}{(}{)}{}{#3,#4} %Plus/minus Iwasawa H^i 
\DeclarePairedDelimiterXPP{\hh}[3]{H_{#1}}{(}{)}{}{#2,#3} %H_i
\DeclarePairedDelimiterXPP{\TateH}[3]{\widehat{\operatorname{H}}^{#1}}{(}{)}{}{#2,#3} %Tate H^i 
\DeclarePairedDelimiter{\roundparenthesis}{(}{)}
\newcommand*{\defect}[1]{\delta_{#1}} %The ``defect'' of injectivity among Selmer groups for the optional curve #1
\newcommand*{\seldim}[2][\multisign]{\rho^{#1}_{#2}} %The common dimension of the dual Selmer in Prop. 5.2; #1 is the sign, #2 the curve
%\DeclareMathOperator{\badpr}{pr_{\raisebox{-.3em}{\tiny$\mathrm{bad}$}}} %The projection of \pmlambda onto the bad components
\DeclareMathOperator{\ppr}{pr_{\raisebox{-.3em}{\tiny$\pprimeset$}}} %The projection of \pmlambda onto the ordinary components
\newcommand*{\resLambda}[1][\Gamma]{\Omega(#1)} %Iwasawa algebra with coefficients in \F_p
\newcommand*{\IwLambda}[1][\Gamma]{\Lambda(#1)} %Iwasawa algebra with coefficients in \Z_p
\newcommand*{\iwlambda}[1][\multisign]{\lambda^{#1}} %Iwasawa lambda-invariant
\newcommand*{\iwmu}[1][\multisign]{\mu^{#1}} %Iwasawa mu-invariant
\newcommand*{\rank}[1][\resLambda]{\operatorname{rk}_{#1}} %Rank over A; default is A=\resLambda
\newcommand*{\corank}[1][\IwLambda]{\operatorname{corank}_{#1}} %Rank over A; default is A=\IwLambda
\newcommand*{\trace}[2]{\operatorname{Tr}^{#1}_{#2}} %The trace map
\newcommand*{\res}[2]{\operatorname{res}_{#1}^{#2}} %cohomological restricition from #1 to #2
\newcommand*{\cores}[2]{\operatorname{cores}_{#1}^{#2}} %cohomological corestricition from #1 to #2
\newcommand*{\NSWpsi}[1]{\psi_{#1}} %The arrow psi in NSW, p430
\newcommand*{\NSWeps}[1]{\varepsilon_{#1}} %The arrow epsilon in NSW, p428 ans423
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%Typographical commands%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand*{\longhookrightarrow}{\lhook\joinrel\relbar\joinrel\rightarrow} %Long injective arrow
\newcommand*{\longtwoheadrightarrow}{\joinrel\relbar\joinrel\twoheadrightarrow}%Long surjective arrow
\newcommand*{\suchthat}{\bigm\vert}
\newcommand{\ibid}{\emph{ibid}.}
\newcommand{\ie}{\emph{i.~e.~}}
\newcommand{\loccit}{\emph{loc.~cit}.~}
\newcommand{\cfr}{\emph{cf}.~}
%
\makeatother
